Bounded commuting projections for multipatch spaces with non-matching interfaces

We present commuting projection operators on de Rham sequences of two-dimensional multipatch spaces with local tensor-product parametrization and non-matching interfaces. Our construction yields projection operators which are local and stable in any $L^p$ norm with $p \in [1,\infty]$: it applies to shape-regular spline patches with different mappings and local refinements, under the assumption that neighboring patches have nested resolutions and that interior vertices are shared by exactly four patches. It also applies to de Rham sequences with homogeneous boundary conditions. Following a broken-FEEC approach, we first consider tensor-product commuting projections on the single-patch de Rham sequences, and modify the resulting patch-wise operators so as to enforce their conformity and commutation with the global derivatives, while preserving their projection and stability properties with constants independent of both the diameter and inner resolution of the patches.

==> macros.tex <==

%\usepackage[right]{showlabels}

%%%%%%%%%%%%  extracting \llangle and \rrangle from MnSymbol package:
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother
%%%%%%%%%%%%



\usepackage[T3,T1]{fontenc}
\DeclareSymbolFont{tipa}{T3}{cmr}{m}{n}
\DeclareMathAccent{\invbreve}{\mathalpha}{tipa}{16}


% macro: personal comments -- choose your favorite color ;)
\definecolor{darkgreen}{rgb}{.1,.5,0}
\providecommand{\martin}[1]{\textcolor{violet}{(Martin: #1)}}
\providecommand{\eric}[1]{ \textcolor{blue}{Eric: #1}}
\providecommand{\yaman}[1]{\textcolor{darkgreen}{(Yaman: #1)}}



% macro: accent for test functions
\newcommand{\test}[1]{\check{#1}}

% macro: accent for dual complex objects on the logical domain
% \newcommand{\dualhat}[1]{\invbreve{#1}}
\newcommand{\dualhat}[1]{\breve{#1}}



% NOTE on bold fonts: it seems that
% \usepackage[bbgreekl]{mathbbol} is enough,
% > then bbm and bm probably not needed
% \usepackage{bbm}
% \usepackage{bm}  % redefines \boldsymbol for better spacings, see http://tex.stackexchange.com/questions/3238/bm-package-versus-boldsymbol
\def\bs{\boldsymbol}
\def\t{\tilde}
\def\wt{\widetilde}
\def\wh{\widehat}

% Poincaré constants
\def\cp{c_{P}}
\def\cph{c_{P,h}}
\def\bcp{\bar c_{P}}
\newcommand{\poplus}{\overset{\perp}{\oplus}}
\def\ualp{\underline{\alpha}}

\newcommand{\perpW}{{\perp_W}}
\newcommand{\perph}{{\perp_h}}

\def\ext{\textrm{ext}}
% \def\frH{\mathfrak{H}}
% \def\frZ{\mathfrak{Z}}
% simple fonts to avoid too many alphabets (for now?)
\def\frB{\mathfrak B}
\def\frH{\mathfrak H}
\def\frZ{\mathfrak Z}

\def\ti{\tilde \imath}
\def\vp{{\varphi}}
\def\ve{{\varepsilon}}
\def\eps{{\epsilon}}

% \def\Nppc{N_{\rm ppc}}

\def\ba{{\bs a}}
\def\bb{{\bs b}}
\def\bc{{\bs c}}
\def\be{{\bs e}}
\def\bsf{{\bs f}}
\def\bg{{\bs g}}
\def\bi{{\bs i}}
\def\bj{{\bs j}}
\def\bk{{\bs k}}
\def\bsm{{\bs m}}
\def\bn{{\bs n}}
\def\bp{{\bs p}}
\def\bq{{\bs q}}
\def\br{{\bs r}}
\def\bu{{\bs u}}
\def\bv{{\bs v}}
\def\bw{{\bs w}}
\def\bx{{\bs x}}
\def\by{{\bs y}}
\def\bz{{\bs z}}

\def\bA{{\bs A}}
\def\bB{{\bs B}}
\def\bC{{\bs C}}
\def\bD{{\bs D}}
\def\bE{{\bs E}}
\def\bF{{\bs F}}
\def\bG{{\bs G}}
\def\bH{{\bs H}}
\def\bI{{\bs I}}
\def\bJ{{\bs J}}
\def\bK{{\bs K}}
\def\bL{{\bs L}}
\def\bM{{\bs M}}
\def\bN{{\bs N}}
\def\bP{{\bs P}}
\def\bQ{{\bs Q}}
\def\bR{{\bs R}}
\def\bS{{\bs S}}
\def\bV{{\bs V}}
\def\bW{{\bs W}}
\def\bX{{\bs X}}
\def\bY{{\bs Y}}
\def\bZ{{\bs Z}}

\def\bell{{\bs \ell}}
\def\btau{{\bs \tau}}
\def\bvp{{\bs \varphi}}
\def\bpsi{{\bs \psi}}
\def\bnabla{{\bs \nabla}}
\def\bLambda{{\bs \Lambda}}
\def\bGamma{{\bs \Gamma}}

\def\hv{{\hat v}}
\def\hx{{\hat x}}
\def\hy{{\hat y}}
\def\dhx{{\partial_\hx}}
\def\dhy{{\partial_\hy}}
\def\hbx{{\hat {\bs x}}}
\def\hbv{{\hat {\bs v}}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}

\def\bfx{{\bf x}}
\def\bfv{{\bf v}}

\def\bfA{{\bf A}}
\def\bfB{{\bf B}}
\def\bfE{{\bf E}}
\def\bfJ{{\bf J}}
\def\bfM{{\bf M}}
\def\bfP{{\bf P}}
\def\bfF{{\bf F}}
\def\bfR{{\bf R}}

\def\bftA{\tilde {\bf A}}
\def\bftC{\tilde {\bf C}}
\def\bftM{\tilde {\bf M}}


% blackboard fonts (eg for number sets)
% \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
\def\AA{\mathbbm{A}}
\def\BB{\mathbbm{B}}
\def\CC{\mathbbm{C}}
\def\DD{\mathbbm{D}}
\def\EE{\mathbbm{E}}
\def\FF{\mathbbm{F}}
\def\GG{\mathbbm{G}}
\def\II{\mathbbm{I}}
\def\JJ{\mathbbm{J}}
\def\KK{\mathbbm{K}}
\def\MM{\mathbbm{M}}
\def\NN{\mathbbm{N}}
\def\PP{\mathbbm{P}}
\def\QQ{\mathbbm{Q}}
\def\RR{\mathbbm{R}}
\def\SS{\mathbbm{S}}
\def\TT{\mathbbm{T}}
\def\VV{\mathbbm{V}}
\def\WW{\mathbbm{W}}
\def\XX{\mathbbm{X}}
\def\YY{\mathbbm{Y}}
\def\ZZ{\mathbbm{Z}}

% \def\one{\mathbbm{1}}

% \def\BB{\mathbb{B}}
% \def\CC{\mathbb{C}}
% \def\DD{\mathbb{D}}
% \def\GG{\mathbb{G}}
% \def\HH{\mathbb{H}}
% \def\II{\mathbb{I}}
% \def\MM{\mathbb{M}}
% \def\NN{\mathbb{N}}
% \def\PP{\mathbb{P}}
% \def\QQ{\mathbb{Q}}
% \def\RR{\mathbb{R}}
% \def\ZZ{\mathbb{Z}}

% % bold blackboard fonts
% % \mathbbm, \mathbbmss or \mathbbmtt with \usepackage{bbm}
% \def\bAA{\mathbbm{A}}
% \def\bCC{\mathbbm{C}}
% \def\bNN{\mathbbm{N}}
% \def\bPP{\mathbbm{P}}
% \def\bRR{\mathbbm{R}}
% \def\bZZ{\mathbbm{Z}}

\def\one{{\mathbbm{1}}}

\def\gl{\mathrm{GL}}

%\usepackage{relsize}
\usepackage{ esint }
\def\fintOm{{\fint_\Omega}}

% \def\cNII{\cN^{\rm {II}}}
% \def\cNI{\cN^{\rm {I}}}
% \def\cRT{\mathcal{RT}}
% \def\cBDM{\mathcal{BDM}}

% \def\vol{{\rm vol}}
% \def\face{{\rm face}}
% \def\edge{{\rm edge}}
% \def\vertex{{\rm vertex}}
% \def\cell{{\rm cell}}



\def\ex{\textrm{ex}}
\def\parts{\textrm{parts}}

\def\corr{\textrm{corr}}
\def\pw{\ensuremath{\mathrm{pw}}} %\textrm{pw}} 

\def\sfA{\mathsf{A}}
\def\sfM{\mathsf{M}}
\def\sfP{\mathsf{P}}
\def\sfT{\mathsf{T}}


\def\Pe{{\sfP^{1}_{h,0}}}
\def\Pm{{\sfP^{0}_h}}

\def\Veh{V^\ve_h}
\def\tVeh{{\t V^\ve_h}}
\def\Vmh{V^\mu_h}
\def\tVmh{{\t V^{\mu}_h}}
\def\Vnuh{V^{\nu}_h}

% \def\DG{{\rm DG}}
% \def\pFE{{p_{\rm fe}}}
% \def\pDG{{p_{\rm dg}}}

\def\intstepn{\int_{t^n}^{t^{n+1}}\mspace{-10mu}}
\def\rmd{\, \textrm{d}} %for integrals
\def\dd{\, \textrm{d}} %for integrals
\def\Dt{{\Delta t}}
\def\Dhx{{\Delta \hx}}
\def\Dhy{{\Delta \hy}}
\def\dt{{\partial_{t}}}
\def\dx{{\partial_{x}}}
\def\dy{{\partial_{y}}}
\def\dtt{{\partial^2_{t}}}

\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqq{\begin{equation*}}
\def\eeqq{\end{equation*}}

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\bigabs}[1]{\big|#1\big|}
\providecommand{\Bigabs}[1]{\Big|#1\Big|}
\providecommand{\Abs}[1]{\left\lvert#1\right\rvert}

\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\bignorm}[1]{\big\|#1\big\|}
\providecommand{\Bignorm}[1]{\Big\|#1\Big\|}
\providecommand{\Norm}[1]{\left\lVert#1\right\rVert}

\def\tb{\hbox{$\|\kern -.09em |$}}
\def\bigtb{\hbox{$\big\|\kern -.09em \big|$}}
\def\Bigtb{\hbox{$\Big\|\kern -.09em \Big|$}}

\providecommand{\tnorm}[1]{\tb#1\tb}
\providecommand{\bigtnorm}[1]{\bigtb#1\bigtb}
\providecommand{\Bigtnorm}[1]{\Bigtb#1\Bigtb}

\providecommand{\sprod}[2]{\langle#1,#2\rangle}
\providecommand{\bigsprod}[2]{\big\langle#1,#2\big\rangle}
\providecommand{\Bigsprod}[2]{\Big\langle#1,#2\Big\rangle}
\providecommand{\ssprod}[2]{\llangle#1,#2\rrangle}

\providecommand{\average}[1]{\{\!\!\{#1\}\!\!\}}
\providecommand{\jump}[1]{[\![#1]\!]}

    % \usepackage{stmaryrd}
    %  \llbracket     1 \rrbracket       \quad
    %  \llparenthesis 2 \rrparenthesis   \quad
    %  \llceil        3 \rrceil          \quad
    %  \llfloor       4 \rrfloor         \quad

\providecommand{\openint}[2]{\mathopen{]}#1, #2\mathclose{[}}
\providecommand{\Openint}[2]{\mathopen{}\mathclose{\left]#1, #2\right[}}

\providecommand{\range}[2]{\llbracket #1, #2 \rrbracket}
\providecommand{\Range}[2]{\left\llbracket #1, #2 \right\rrbracket}

% \mathopen{}\mathclose{\left]...\right[}


\newcommand\blue[1]{{\color{blue} #1}}
\newcommand\purple[1]{{\color{purple} #1}}

\providecommand{\note}[1]{{\bf [note: #1]}}
\providecommand{\todo}[1]{{\bf To do}: {\em #1 }}

\def\blankfirst{\phantom{V^0} }
\def\blanksecond{\phantom{ \{ } } %\hspace*{-5pt}}
\def\bbb{\phantom{\big|} }
\def\bBb{\phantom{\Big|} }


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\Int}{int}

\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\gap}{gap}

\DeclareMathOperator{\sign}{sign}

\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rg}{range}
\DeclareMathOperator{\Dom}{Dom}

\DeclareMathOperator{\tbcurlh}{\widetilde \bcurl_{\it h}}
\DeclareMathOperator{\tcurlh}{\widetilde \curl_{\it h}}
\DeclareMathOperator{\bcurlh}{\bcurl_{\it h}}
\DeclareMathOperator{\curlh}{\curl_{\it h}}
\DeclareMathOperator{\tcurlha}{\widetilde \curl_{\it h}^{\it a}}

\DeclareMathOperator{\curl}{curl}
\DeclareMathOperator{\bcurl}{{\bf curl}}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\bgrad}{{\bf grad}}

\DeclareMathOperator{\tgrad}{\widetilde \grad}
\DeclareMathOperator{\tcurl}{\widetilde \curl}
\DeclareMathOperator{\tDiv}{\widetilde \Div}

\DeclareMathOperator{\hgrad}{\widehat \grad}
\DeclareMathOperator{\hcurl}{\widehat \curl}
\DeclareMathOperator{\hDiv}{\widehat \Div}

% black-board sans serif
% \mathbb require \usepackage ??  [bbgreekl]{mathbbol} of {upgreek} ??
\newcommand{\mat}[1]{\mathbb{#1}}
\def\matd{\mathbb{d}}
\def\matr{\mathbb{r}}
\def\matA{\mathbb{A}}
\def\matB{\mathbb{B}}
\def\matC{\mathbb{C}}
\def\matD{\mathbb{D}}
\def\matF{\mathbb{F}}
\def\matG{\mathbb{G}}
\def\matH{\mathbb{H}}
\def\matI{\mathbb{I}}
\def\matJ{\mathbb{J}}
\def\matK{\mathbb{K}}
\def\matL{\mathbb{L}}
\def\matM{\mathbb{M}}
\def\matN{\mathbb{N}}
\def\matP{\mathbb{P}}
\def\matR{\mathbb{R}}
\def\matS{\mathbb{S}}
\def\matT{\mathbb{T}}
\def\matW{\mathbb{W}}
\def\matX{\mathbb{X}}
\def\matZ{\mathbb{Z}}
\def\matLambda{\mathbb{\Lambda}}

% arrays of stacked quantities (dim = numerical parameter)
\newcommand{\arr}[1]{{\bs{\mathsf{#1}}}}
\newcommand\arre{{\bs{\mathsf{e}}}}
\newcommand\arrg{{\bs{\mathsf{g}}}}
\newcommand\arrB{{\bs{\mathsf{B}}}}
\newcommand\arrD{{\bs{\mathsf{D}}}}
\newcommand\arrE{{\bs{\mathsf{E}}}}
\newcommand\arrH{{\bs{\mathsf{H}}}}
\newcommand\arrJ{{\bs{\mathsf{J}}}}
\newcommand\arrU{{\bs{\mathsf{U}}}}
\newcommand\arrV{{\bs{\mathsf{V}}}}
\newcommand\arrW{{\bs{\mathsf{W}}}}
\newcommand\arrX{{\bs{\mathsf{X}}}}
\newcommand\arrY{{\bs{\mathsf{Y}}}}
\newcommand\arrZ{{\bs{\mathsf{Z}}}}
\newcommand\arrLambda{{\bs{\mathsf{\Lambda}}}}
\newcommand\arrsigma{{\bs{\mathsf{\sigma}}}}

\newcommand\uvec{{\be}}

\usepackage{mathrsfs}
\def\scrc{\mathscr{c}}
\def\scre{\mathscr{e}}
\def\scrf{\mathscr{f}}
\def\scrC{\mathscr{C}}
\def\scrE{\mathscr{E}}
\def\scrF{\mathscr{F}}
\def\scrP{\mathscr{P}}
\def\scrV{\mathscr{V}}

% grid nodes, edges, faces and cells
\newcommand\ttc{{\mathtt{c}}}
\newcommand\tte{{\mathtt{e}}}
\newcommand\ttf{{\mathtt{f}}}
\newcommand\ttg{{\mathtt{g}}}
\newcommand\ttj{{\mathtt{j}}}
\newcommand\ttn{{\mathtt{n}}}
\newcommand\ttv{{\mathtt{v}}}
\newcommand\ttx{{\mathtt{x}}}


\newcommand\ttC{{\mathtt{C}}}
\newcommand\ttE{{\mathtt{E}}}
\newcommand\ttF{{\mathtt{F}}}
\newcommand\ttG{{\mathtt{G}}}
\newcommand\ttN{{\mathtt{N}}}


\newcommand\gx{\bx}
%\newcommand\gx{{\bf{\texttt{x}}}}
% \def\gx{\bs{\ttx}}  % grid x



% interior products, continuous and discrete
\newcommand{\ip}[2]{i^{#1}_{#2}}
\newcommand{\tip}[2]{\tilde \imath^{#1}_{#2}}
\newcommand{\hiph}[2]{\hat \imath^{#1}_{h,#2}}
\newcommand{\iph}[2]{i^{#1}_{h,#2}}
\newcommand{\tiph}[2]{\tilde \imath^{#1}_{h,#2}}
% alternate notation:
%\newcommand{\ip}[2]{\imath^{#1}_{\uvec_{#2}}}
%\newcommand{\iph}[2]{I^{#1}_{h,\uvec_{#2}}}

